Deep Learning-based Real-time Smartphone Pose Detection for Ultra-wideband Tagless Gate

As commercial interest in proximity services increased, the development of various wireless localization techniques was promoted. In line with this trend, Ultra-wideband (UWB) is emerging as a promising solution that can realize proximity services thanks to centimeter-level localization accuracy. In addition, since the actual location of the mobile device (MD) on the human body, called pose, affects the localization accuracy, poses are also important to provide accurate proximity services, especially for the UWB tagless gate (UTG). In this paper, a real-time pose detector, termed D3, is proposed to estimate the pose of MD when users pass through UTG. D3 is based on line-of-sight (LOS) and non-LOS (NLOS) classification using UWB channel impulse response and utilizes the inertial measurement unit embedded in the smartphone to estimate the pose. D3 is implemented on Samsung Galaxy Note20 Ultra (i.e., SMN986B) and Qorvo UWB board to show the feasibility and applicability. D3 achieved an LOS/NLOS classification accuracy of 0.984, and ultimately detected four different poses of MD with an accuracy of 0.961 in real-time.

==> README.tex <==
introduction
1) 왜 pose classification이 필요한지 
2) UWB를 활용한 최근 application이 어떤 것들이 있는지 Tagless Gate 
3) 우리가 가정하는 시나리오는 어떤 시나리오인지

Diverse application and reference
1. Tagless Gate
https://www.nxp.com/video/uwb-minutes-uwb-for-access-control:UWB-MINUTES-ACCESS-CONTROL
2. Digital Car Key (BMW)
https://www.bmw.com/en/innovation/bmw-digital-key-plus-ultra-wideband.html
3. NEAR project
https://www.nxp.com/company/about-nxp/nxp-collaborates-with-ing-and-samsung-to-pilot-industrys-first-uwb-based-peer-to-peer-payment-application:NW-NXP-COLLABORATES-WITH-ING-AND-SAMSUNG-TO
 

Strength: 
1.Qorvo와 연결해서 real-time으로 수행 (On Android)
2.Real-time으로 구현하는것이 어떤부분에서 challenging 한지 (USB serial로 데이터를 전송 받아야 하는데 그냥 printf 한다고 되는게 아니다)
3. Qorvo보드 부분과 스마트폰 부분 모두 구현을 하였다

Weakness: 
1. Google API만 제공된다면 단일기기로 수행가능 (Google API의 현상태 체크 필요)
2. 4가지 pose 이외의 더 다양한 pose를 구분할 필요가 있음 (future work으로 작성 가능)

Conclusion
1. UWB의 CIR을 통해서 LOS/NLOS를 구분하고 그결과를 바탕으로 동일 시간에서의 IMU 센서를 바탕으로 각각의 POSE를 classification 하는 문제로 단순화하였음.

Future work
1. Pose classification 기반으로 실제 Tagless Gate, Digital Car Key에 직접 적용해서 performance를 확인하는 부분이 남아있다.
2. 
